Preliminary Exploration of Formula Embedding for Mathematical Information Retrieval: can mathematical formulae be embedded like a natural language?

While neural network approaches are achieving breakthrough performance in the natural language related fields, there have been few similar attempts at mathematical language related tasks. In this study, we explore the potential of applying neural representation techniques to Mathematical Information Retrieval (MIR) tasks. In more detail, we first briefly analyze the characteristic differences between natural language and mathematical language. Then we design a "symbol2vec" method to learn the vector representations of formula symbols (numbers, variables, operators, functions, etc.) Finally, we propose a "formula2vec" based MIR approach and evaluate its performance. Preliminary experiment results show that there is a promising potential for applying formula embedding models to mathematical language representation and MIR tasks.

==> content/experiment.tex <==
% \vspace{-2ex} \section{Experiment}

% \subsection{Dataset and Experiment Setting}

% We tested the proposed approach in a ``Chinese-to-English'' recommendation task. Our goal was to recommend English citations for a given Chinese paper's abstract with its Chinese citation relations. For this experiment, we collected 14,631 Chinese papers (in computer science) from the Wanfang digital library and 248,893 English papers from the Association for Computing Machinery (ACM) digital library. There were 750,557 English-cite-English relations, 11,252 Chinese-cite-Chinese relations, 27,101 Chinese-cite-English relations, and 12,403 English papers had been cited by 7,900 Chinese papers. Using machine translation and language modeling, we generated 158,000 cross-language semantic matching relations (from Chinese to English) for cross-language semantic enrichment. 





% For cross-language citation recommendation evaluation, we generated test and candidate collections by following method: (1) randomly selected 10\% papers from 7,900 Chinese papers that have cross-language citation relations to English corpus; (2) removed all cross-language citation relations from selected Chinese papers (Chinese citation relations could be kept); (3) the processed 10\% of papers were used as a test collection, all English papers cited by the Chinese papers in the test collection were used as candidate collection. To avoid evaluation bias, 10-fold cross-validation was applied. We recommended English citations from the candidate collection. In this study, we used a 0-1 relevant score for evaluation. For example, if a candidate paper was cited by the target testing paper, the relevant score was 1, otherwise it was 0.

% \vspace{-2ex} \subsection{Experiment Results}
% We evaluated the performance of proposed PRCC method against the following strong baseline algorithms\footnote{Because of the space limitation, we cannot provide more detailed baseline information. The detailed descriptions about baselines will be available in the project website (URL is omitted for review)}: (1) Embedding Transformation (EF) \cite{mikolov2013exploiting}; (2) Item-based Collaborative Filtering (CF$_{I}$); (3) Popularity-based Collaborative Filtering (CF$_{P}$); (4) Machine Translation by Google Translation API + Language Model with Dirichlet smoothing (MT+LM); (5) Node2vec node embedding \cite{grover2016node2vec} based on Citation Network (N2C$_{C}$).

% \begin{table}[htbp]
% \centering
% \footnotesize
% \caption{Measures of different cross-language citation recommendation algorithms}\vspace{-2ex} 
% \label{tab:result}
% \begin{threeparttable}
% \begin{tabular}{l l l l l }
% \hline
% \textbf{Algorithm} & \textbf{NDCG@10} & \textbf{P@10} & \textbf{MAP} & \textbf{MRR} \\ \hline
% EF        & 0.0176 & 0.0072 & 0.0185 & 0.0300  \\ 
% CF$_{I}$  & 0.0980 & 0.0330 & 0.0815 & 0.1290  \\ 
% CF$_{P}$  & 0.0041 & 0.0026 & 0.0125 & 0.0090  \\ 
% MT+LM     & 0.3404 & 0.1225 & 0.2831 & 0.3312  \\ 
% N2C$_{C}$ & 0.2289 & 0.0938 & 0.1983 & 0.2550  \\ 
% \textbf{PRCC}       & \textit{\textbf{0.3908}}\textsuperscript{\dag\dag\dag} & \textit{\textbf{0.1543}}\textsuperscript{\dag\dag\dag} & \textit{\textbf{0.3312}}\textsuperscript{\dag\dag\dag} & \textit{\textbf{0.4411}}\textsuperscript{\dag\dag\dag}  \\ \hline
% \end{tabular}  
% \begin{tablenotes}
%     \footnotesize
%     \item Significant test: PRCC vs. Other algorithms; \textsuperscript{\dag}$p < 0.01$, \textsuperscript{\dag\dag}$p < 0.001$, \textsuperscript{\dag\dag\dag}$p < 0.0001$
%     \end{tablenotes}
% \end{threeparttable}
% \end{table}\vspace{-2ex} 

% As Table \ref{tab:result} shows, PRCC ($\alpha = 0.25$) achieves best performance ($p<0.0001$) in all evaluation metrics, and content-based approach ``MT+LM'' gets the second best performance. Node2vec (based on citation network) gets the third best.

% When we merge the semantic matching probability and citation probability, parameter $\alpha$ is an important parameter. It controls the contributions from citation and content semantic. Based on a randomly selected testing collection (10\%), we tried different $\alpha$ value for content and citation merging. The recommendation performance under different $\alpha$ is shown in Figure \ref{fig:alpha}.

% As Figure \ref{fig:alpha} shows, under different $\alpha$, the performance measured by different metrics shows similar changing trends: when $\alpha$ increases from 0.25 to 1, the performance declines slightly; when $\alpha$ increases to 2, the performance declines sharply and keeps a slight decline when $\alpha$ increases to 4.


% \begin{figure}[htbp]\centering
%  	\includegraphics[width=0.9\columnwidth]{pics/alpha_2.png} \vspace{-2ex} 
%  	\caption{Recommendation performance under different $\alpha$}
%  	\label{fig:alpha}
% \end{figure}\vspace{-2ex} 

==> content/review.tex <==
% \vspace{-2ex} \section{RELATED WORK}\label{review}

% Citation recommendation aims to recommend a list of citations (references) based on the similarity between the recommended papers and user profiles or samples of in-progress text. For instance, He et al.~\cite{he2010context} proposed a probabilistic model to compute the relevance score based on contexts of a citation and its abstract. Jiang et al.~\cite{jiang2015chronological} generated a heterogeneous graph with various relations between topics and paper, and a supervised random walk was used for citation recommendation. From bibliographic viewpoint, Shi, Leskovec, and McFarland~\cite{citing-impact} developed citation projection graphs by investigating citations among publications cited by a given paper. Collaborative filtering algorithm can also be used for recommending citation papers \cite{mcnee2002recommending}. However, all of the prior studies focused on monolingual citation recommendation and cannot be directly used for cross-language citation recommendation. 

% %McNee et al.  build a rating matrix based on the citation web to recommend scientific papers. 

% Intuitively, translation-based models can be addressed for cross-language recommendation. Recently, word embedding is a powerful approach for content representation \cite{mikolov2013efficient}, which can discover distributed representations of words and capture the semantic similarity between the words. Mikolov et al. \cite{mikolov2013exploiting} transformed one language's vector space into the space of another by utilizing a linear projection with a transformation matrix $W$. This approach is effective for word translation, but the translation effect for scholarly text has not yet been demonstrated. Tang et al.~\cite{tang2014cross} proposed bilingual embedding algorithms, which were efficient for cross-language context-aware citation recommendation task. However, they ignored the important citation relations in their work. Following the main idea of word embeddings, Grover and Leskovec \cite{grover2016node2vec} proposed node2vec for learning continuous feature representations of nodes in networks. But, node2vec has two limitations for cross-language citation recommendation. First, node2vec, aiming for learning the representations of connected nodes, can hardly learn the representation of ``isolate'' paper node with no citation relations to/from itself. Second, if we apply node2vec based on citation networks, it will lose content information, and the textual content can be very important to citation recommendation. In this study, we will address these problems and propose a novel method to learn a mapping of publication to a low-dimensional joint embedding space for both content and citation information. 
